New (TH)GEM coating materials characterised using spectroscopy methods

In this work GEM and single-hole Thick GEM structures, composed of different coating materials, are studied. The used foils incorporate conductive layers made of copper, aluminium, molybdenum, stainless steel, tungsten and tantalum. The main focus of the study is the determination of the material dependence of the formation of electrical discharges in GEM-based detectors. For this task, discharge probability measurements are conducted with several Thick GEM samples using a basic electronics readout chain. In addition to that, optical spectroscopy methods are employed to study the light emitted during discharges from the different foils. It is observed that the light spectra of GEMs include emission lines from the conductive layer material. This indicates the presence of the foil material in the discharge plasma after the initial spark. However, no lines associated with the coating material are observed while studying spark discharges induced in Thick GEMs. It is concluded that the conductive layer material does not play a substantial role in terms of stability against primary discharges. However, a strong material dependence is observed in the case of secondary discharge formation, pointing to molybdenum coating as the one providing increased stability.

==> ToDo.tex <==
\section{ToDo}
This is a ToDo list for all the sections of the paper:

%% Title %%
\subsection{title page}
+ Finalize paper name
    - Done: "Search for new (TH)GEM coating materials using spectroscopy methods"
+ Determine author list
    -Done
+ Gather author info
    -Done

%% Abstract %%
\subsection{abstract}
+ write abstract
    -Done

%% Introduction %%
\subsection{intro}
+ Determine introduction structure
    - Done: 1. General GEM intro
            1.1. Search for new materials
            1.2. Spectroscopy studies with GEM discharges
+ Find citations
    - Done
+ Finish writing introduction
    - Done

%% Used GEM structures %%
\subsection{used GEMs}
+ Determine section structure
    - Done: 2.1 Properties of the used foils
                - THGEM/ GEM geometry
                - Material properties and motivating the decision behind used materials
            2.2 Production Methods
+ Take better foil photos
    -Done
+ Make THGEM/GEM geometry sketch
    -Not needed
+ Talk to Rui/ Simon for 2.2
    -Done
+ Find citations
    -Done

%% Experimental setup and measurement methods for discharge studies %%
\subsection{experimental setup}
+ Determine section structure
    -Done
+ Improved setup sketch
    -Done
+ Find citations
    -Done

%% Results %%
\subsection{results}
+ Update all plots to calibrated ones
    -Done
+ Determine section structure
    -Done
+ Finalizing which plots will be shown
    - Done: ° Gas comparison with Cu GEM
            ° Primary vs secondary
            ° Cu GEM vs Al GEM
            ° GEM vs THGEM
            ° Exotic THGEMs
+ Find citations
    -Done

%% Discussions %% 
\subsection{discussions}
+ Find citations
    -Done
+ Conclude: What are our findings what are open questions?
    -Done
+ Write discussions
    -Done
+ Find possible explanations for molybdenum anomaly
    -Done

%% References %%
\subsection{references}
+ Find citations
+ Make references.bib

%% Comments in introduction

%\blue{Either we start with GEM description, which i do not think is necessary, or we go directly to discharges, which, in spite of the title, are the topic of this paper...}\\[1ex]

%\subsection{Discharges in GEM detectors}
%Although studied since the first development of the micro pattern gaseous detectors in late 80's.
%When they occur, discharges in GEMs lead to the short-term blinding of the detector and can even damage the involved detector components \cite{merlin2016study}. Thus, it is crucial to understand these events on a microscopic basis and to develop methods to mitigate the formation of such breakdown events. Currently, many effective discharge mitigation strategies have been developed. Similarly, there have also been significant advancements concerning our understanding of the physical mechanisms leading to the formation of discharges in GEMs \cite{peskov2012advances,gasik2017charge}. To this point, a distinction has to be made concerning the different types of discharges that are observed to occur in GEM and THGEM detectors.

%The most prevalent discharge type, referred to as primary GEM discharge, is attributed to a spark that occurs within GEM holes, leading to the momentary shorting of the two sides of the involved GEM foil. It was shown that these primary discharges can be mitigated with various methods \cite{bachmann2002discharge}. These include among others, operating the detector with a quencher-rich gas mixture or optimizing the RC components of the high-voltage system \cite{gasik2014development}. Furthermore, the formation and evolution of primary discharges have been simulated and even the primary discharge stability of detectors incorporating different geometrical and gas properties can be modeled numerically \cite{peskov2009research,gasik2017charge}. Based on these methods, the current understanding dictates that when the charge density inside a GEM hole exceeds a certain limit (caused by an increased number of charge carriers entering the hole within a given period) the formation of a streamer is triggered causing the breakdown  \cite{gasik2017charge}.



%Recently, a study was conducted to measure the time evolution of the light emission during GEM discharges using a very high-speed camera \cite{utrobicic2019studies}. This optical approach yielded new insights into the long time delay between primary and secondary discharges and into the processes that occur during this transition period. It was shown that studying GEM discharges optically can become a novel tool for probing the physical mechanisms leading to discharge formation. 

%So far, there have been no systematic studies focusing on the color spectra of the emitted light from discharges in GEMs. 
% The primary discharge 

% GEM electrodes, which
% in turn facilitates the thermionic emission of further electrons
% upon ion bombardment and infra-red radiation. 

% heats GEM electrodes allowing for thermionic emission of secondary electrons. In addition, with high enough number of charges created in a primary discharge, ionization and excitation processes occur in the gap below discharging GEM. Ions stemming from the ionization process 

% Ionization ions drifting back towards the bottom side of the foil, cause further emmission of electrons 

% enough electronos t cause further gas ionisatin and exitation in the gap below GEM 


% causing ions drifting towards the bottom GEM electrode (being the cathode in the described process). 

% In addition, the primary discharge heats it heats GEM electrodes which
% in turn facilitates the thermionic emission of further electrons
% upon ion bombardment and infra-red radiation. 



% produces enough electrons to cause further ionisation in the gap below GEM. 


% In this work ....

% If enough charge is produced
% in the primary discharge, further ionisation and excitation produce
% thermionic emission of electrons from the cathode, which
% is in turn heated by ion bombardement. This process is selfsustained
% until eventually massive electron emission results in
% the breakdown of the gap.

% Based on the measurements and simulations presented in
% this work, we propose a mechanism responsible for the occurrence
% of secondary discharges: upon the primary discharge, a
% sucient amount of electrons are produced that can ionise and
% excite the gas in the concerned gap. The primary discharge
% produces also a certain heat load on the GEM electrodes, which
% in turn facilitates the thermionic emission of further electrons
% upon ion bombardment and infra-red radiation. 


% in which the thermionic emission from the heated cathode was proposed as a necessary source of secondary electrons, feeding the plasma which may eventually transform into a spark . It is still 




%now mitigation strategies (briefly) and then...

%here: why doo we want to study different materials? To see if spectroscopy will shed some light, measuree temperature of a discharge and possible correlatioons with secnodary prbabnility.



%Still, there are unanswered questions around the topic of discharges in GEMs, especially concerning the less common type of GEM discharges called delayed secondary discharges. In contrast to primary discharges, secondary discharges do not occur within GEM holes. They are attributed to breakdowns propagating in the gap between neighboring GEM foils and/or the read-out electrode. Due to the potential consequences on the read-out electronics, these events are in general much more dangerous for the detector. Motivated by this, mitigation methods for secondary discharges have also been widely studied establishing improved detector design strategies \cite{lautner2019high}. 

%Yet, the origin of these breakdown events is currently not fully understood. Although there are many hypotheses, the exact conditions inducing secondary discharges can't be modeled microscopically. This is mainly due to one observed behavior. Secondary discharges can, under certain circumstances, occur after a very long time delay (\SIrange{1}{100}{\micro s}) after the triggering primary discharge. These time scales are considerably larger than the values expected for discharge propagation processes such as VUV-photon emission \cite{peskov2009research}, hence this scenario is not very plausible as the cause of the secondary discharges. Another hypothesis, currently very popular in the GEM discharge community, explains the formation of secondary discharges with thermionic electrons (emitted from the GEM foil cathode surface after it is heated by the primary discharge) drifting towards the consequent anode electrode \cite{deisting2019secondary,utrobicic2019studies}. Whereas this explanation is satisfactory to describe the observed time delay, it lacks consistency when other experimental observations are also taken into consideration. In particular, it is not consistent with the unperturbed occurrence of secondary discharges even when the applied electric field in the involved gap is inverted. 
%
%Thus, some additional, yet unknown, processes are possibly involved in delayed secondary discharge formation. The here presented work aims to unveil new insights concerning the formation mechanisms of delayed secondary discharges in GEM detectors. We propose a new approach to use spectroscopy for investigating the light emitted during and before secondary discharge formation. Also, to further investigate the thermionic emission hypothesis, we focus on the influence of different (TH)GEM materials on the creation of such violent events.  






%There are several standard measures to minimize sparking probability and the damage caused by occasional sparks in MPGDs. These are:
%A.	using several structures stacked on top of each other to distribute the avalanche charges among many amplification stages [1];
%B.	dividing the active surface of the detector into several smaller, electrically isolated parts, reducing the discharge energy [1];
%C.	using protections (decoupling) resistors in series with the detector electrodes to reduce the discharge current and implementation of spark-protected front-end electronics;
%D.	implementation of resistive electrodes instead of the traditional metallic ones. Such detectors (e.g. resistive MICROMEGAS, resistive µRWELL, resistive GEM) are hybrids between RPC (Resistive Plate Chamber) and MPGD detectors [4]. The advantage of this solution, besides the reduced discharge probability, is that only the region closest to a spark is affected by the discharge while the rest of the detector area remains active. They also protect the readout electronics.



%here only why new materials and spectroscopy, these nice paragraphs should go to the next chapter and experimental methods.

%\subsection{Search for new materials}
%GEM and THGEM electrodes are usually made of copper. This material choice is generally motivated by the available know-how in producing foil-like structures predominantly with copper within the PCB manufacturing community. Recently, a lot of effort has been invested in producing GEM structures using different materials to study their effects on detector performance. These new materials include DLC (diamond-like carbon) \cite{song2020DLCTHGEM}, ceramic \cite{zhou2020ceramic} and gold \cite{koike2011gold}. 



%\subsection{Spectroscopy studies on GEM and THGEM discharges}
%Over the years there has been an extensive effort to study discharge formation in GEM detectors due to them directly limiting detector performance. Most of these studies have aimed to understand the movement of the free charges inside and around the GEM holes during discharges by probing the electrical signal the discharges induce inside the detector \cite{bachmann2002discharge, peskov2009research}. This approach has yielded many results and constitutes the basis of our understanding of primary discharge formation in GEMs. Still, it is currently not sufficient to explain the secondary discharge phenomenon \cite{deisting2019secondary}. Furthermore, there are so far not many systematic studies concerning the properties of the light emitted during discharges in GEM detectors. 

